Information Bottleneck on General Alphabets

We prove rigorously a source coding theorem that can probably be considered folklore, a generalization to arbitrary alphabets of a problem motivated by the Information Bottleneck method. For general random variables $(Y, X)$, we show essentially that for some $n \in \mathbb{N}$, a function $f$ with rate limit $\log|f| \le nR$ and $I(Y^n; f(X^n)) \ge nS$ exists if and only if there is a random variable $U$ such that the Markov chain $Y - X - U$ holds, $I(U; X) \le R$ and $I(U; Y) \ge S$. The proof relies on the well established discrete case and showcases a technique for lifting discrete coding theorems to arbitrary alphabets.

==> custom_draft.tex <==

\newcommand{\longversion}{\set{\pversion}{long}}
\newcommand{\shortversion}{\set{\pversion}{short}}

\newenvironment{vlong}{
  \ifthenelse {\equal{\pversion}{short}} {\newenvironment{vshort}{
  \ifthenelse {\equal{\pversion}{long}} {


==> custom_versions.tex <==

\RequirePackage{substr}
\makeatletter
\@ifclassloaded{beamer}{}{
  \RequirePackage{environ}
}

\newif\iflong
\newif\ifshort
\newif\ifprintversion

\NewEnviron{vlong}{%
  \iflong
    \BODY
  \fi
}
\NewEnviron{vshort}{%
  \ifshort
    \BODY
  \fi
}

\longtrue
\printversionfalse

\newcommand{\shortversion}{\longfalse \shorttrue}
\newcommand{\longversion}{\longtrue \shortfalse}
\newcommand{\printversion}{\printversiontrue}

\IfSubStringInString{\detokenize{shortversion}}{\jobname}
{
  \shortversion
}{}

\IfSubStringInString{\detokenize{printversion}}{\jobname}
{
  \printversion
}{}



